Dexterous In-hand Manipulation by Guiding Exploration with Simple Sub-skill Controllers

Recently, reinforcement learning has led to dexterous manipulation skills of increasing complexity. Nonetheless, learning these skills in simulation still exhibits poor sample-efficiency which stems from the fact these skills are learned from scratch without the benefit of any domain expertise. In this work, we aim to improve the sample efficiency of learning dexterous in-hand manipulation skills using controllers available via domain knowledge. To this end, we design simple sub-skill controllers and demonstrate improved sample efficiency using a framework that guides exploration toward relevant state space by following actions from these controllers. We are the first to demonstrate learning hard-to-explore finger-gaiting in-hand manipulation skills without the use of an exploratory reset distribution. Video results can be found at https://roamlab.github.io/vge

==> text/literature.tex <==
Imitation learning is commonly analyzed via regret minimization. The availability of an expert policy clearly makes it possible to define some estimate of optimal value. The learner only attempts to imitate the oracle’s behavior without any notion of the task loss function.
\begin{itemize}
    \item IL from fixed demonstrations
    \item IL from experts
\end{itemize}
What are the categories of related work that we want to use? The first category of related work is Imitation Learning and closely related to this category is Interactive Imitation Learning. \textcite{Cheng2020-wo} propose MAMBA a policy improvement method based imitation of multiple experts. However, the experts used are unrealistic as they are partially trained policies. 

The general paradigm of querying expert is called Interactive Imitation Learning. Direct Policy Learning is a class of algorithms for this paradigm. 

\textcite{Daume_undated-bg} use contextual bandit algorithm oracle to trade-off exploration and exploitation.  We do something very similar? They use Boltzmann exploration for constructing the oracle. So our exploration is also Boltzmann Exploration. Our method may be one of the first at combining multiple experts through Boltzmann exploration. The rollout policy $\pi_{mix}$ assigns fixed probabilities of sampling between a reference policy (the sub-optimal expert) $\pi_{ref}$ policy and learner policy $\pi_{learn}$. The contextual bandit oracle. This uses the RIRO framework. The episode rollout consists of two parts. In the first part the actions are selected by $pi_{mix}$ and in the second part the actions are selected by a contextual bandit oracle. RIRO rollouts aren't efficient for highly suboptimal experts.

\textcite{Sun2018-zu} proposed  THOR (Truncated HORizon Policy Search) can access a cost-to-go oracle \cite{Ross2014-qk}, providing additional information
about the long-term effects of learner decisions. This oracle is used to reshape rewards and policy gradients are computed w.r.t to the reshaped rewards. Assuming access to the cost-to-go of the oracle has two main issues. First, the cost-to-go for the oracle must be sufficiently accurate w.r.t to the optimal policy which is really hard. Estimating the cost-go-to of the expert also holds little meaning as these skills have almost zero returns.

\textcite{Ranzato2015-tk} used data as demonstrator (DAD) for sequence prediction for text generation tasks.

\textcite{Beliaev2022-vz} address the problem of combing demonstrations from multiple experts where the quality of the demonstrations can vary between the demonstrator. They learn a model to predict the quality of the expert demonstrations given embedding for the state and the demonstrators. 
\textcite{Ross2014-rr} proposed AggreVaTe. This is one of the key algorithms that MAMBA builds on for multiple experts. AggreVaTe is the first algorithm to notice that prior algorithms didn't benefit from information about the cost-of-actions. Hence, AggreVaTe is the first method to use the cost/value of the action in the context of Interactive Imitation Learning. This work suggested a broad family of policy iteration algorithms that unified imitation and reinforcement learning. (THOR also does this too, maybe it is not the first). "Iterative training procedures which interleave execution and training have impressive performance".  They are the first to propose RIRO rollout? 

\textcite{He_undated-tx} SEARN. SEARN, does reason about cost-to-go, but uses rollouts from the current policy which can be impractical for imitation learning. SEARN additionally requires the use of stochastic policies. \textit{Why is it impractical for imitation learning?}

We should also compare with RIRO rollout strategy. 
It looks like our method maybe the first properly scalable method for multi-expert imitation learning. The prior methods have used either online learning and don't benefit from the recent advances in deep RL. 

\textcite{Kurenkov2019-ye}(2019) proposed AC Teach. Our work is most similar to this work. Among the action proposals from various policies, the best action is the one that has highest probability of increasing the Q-value. They also have a decay parameter to achieve consistency between actions selected. We differ from them in the following ways. (1) We use a minimum of two Q-networks instead of Bayesian Q-network. This allows us to compatible with off-policy that don't use a bayesian critic.  (2) We use a softmax instead of greedy max selection between proposed actions. (Internal note: We should implement this. It is easy and has a decent chance that it won't work, atleast on our problem)

==> text/results_backup.tex <==
\subsection{Learning from single-expert}

First we preset our method on learning from a single expert using each of the previously described experts one at a time. For comparison, we also  use the method with the following baselines methods.
\begin{figure}[h]
\centering
% \includegraphics[width=0.5\textwidth]{figs/sac_flagship.jpg}
% \includegraphics[width=0.5\textwidth]{figs/SAC_cube_Psoe_vs_random_initial_states.png}
\includegraphics[width=0.4\textwidth, height=0.25\textwidth]{example-image}
\caption{Single expert experiments with SAC. \todo{We need the following curves in a single plot. 1. Ours 2. Ours w/o BC 2. FS 3. NE  4. NE + SGS}}
\label{fig:sing-expert-SAC}
\end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=0.5\textwidth]{figs/sac_flagship.jpg}
% \includegraphics[width=0.5\textwidth]{figs/SAC_cube_Psoe_vs_random_initial_states.png}
\includegraphics[width=0.4\textwidth, height=0.25\textwidth]{example-image}
\caption{Single expert experiments with TD3. \todo{We need the following curves in a single plot. 1. Q-value with finger gaiting expert  2. Fixed schedule with finger-gaiting expert}}
\label{fig:sing-expert-TD3}
\end{figure}


Our results that first we are able to learn with finger-gaiting expert while the in-grasp manipulation and contact switching expert do not help in learning the policy when used by itself. While \textit{FS} baseline methods results in learning a policy, we found that it is not robust across seeds with a 20\% success rate. However, our method robust to variation in seeds with a success rate of about 90\%. These results have the same trend with both SAC and TD3. 

\subsection{Learning from multiple experts}

In this section, we show our key result for learning finger-gaiting in-hand manipulation from multiple experts. We will use the in-grasp manipulation expert and contact switching expert simultaneously.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth, height=0.25\textwidth]{example-image}
% \includegraphics[width=0.5\textwidth]{figs/SAC_cube_Psoe_vs_random_initial_states.png}
\caption{\todo{Learning from multiple expert. 1. Ours, turning expert + switching expert 2. Ours, + finger-gaiting expert. 2. Q-value + turning expert + switching expert  3. Ours Ideally, we will find that multi-expert approach outperforms using a single-expert.} }
\label{psoe_decay_vs_random_initial_states}
\end{figure}


\subsection{Ablations}

\textit{Without BC loss}.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth, height=0.25\textwidth]{example-image}
% \includegraphics[width=0.5\textwidth]{figs/SAC_cube_Psoe_vs_random_initial_states.png}
\caption{\todo{Taking out the BC loss should show worse performance} }
\label{psoe_decay_vs_random_initial_states}
\end{figure}


% SAC vs TD3
% 1. Ours + expert1
% 2. Ours + expert2
% 3. Ours + expert3
% 4. Ours + expert1 + expert2
% 5. Ours w/o BC + expert 1
% 6. Ours w/o BC + expert 2
% 7. Ours w/o BC + expert 3
% 8. Ours w/o BC + expert 1 + expert 2
% 9. FS + expert1
% 10. FS + expert2 
% 11. FS + expert3 
% 12. FS + expert1 + expert2
% 





% \textbf{Only Switching and Turning}


% According to the results of Guided Exploration with the turning controllers, the controller guides the exploration to a local optima. This "false guidance" is difficult to forsee because because the action space has 15 dimentions and is not intuitive to humans. Unlike finger switching, turning is a relatively easy task for RL to achieve and the state space for successful turning is large. However, only a portion of it can lead to successful gaiting. In contrast, it seems that the state space for successfull switching may not be as large, and will more often lead to succesfull gaiting. Figure \ref{local_optima} attempts to illustrate this situation.



% \subsection{Finger-gaiting in-hand manipulation}

% In this task, the goal is to continuously rotate an about z-axis via finger gaiting. We consider this problem both in 2D and 3D as shown in Figure \ref{hand_model}. The robotic hand has identical fingers located symmetrically from the center.  In 2D, the hand has 4 fingers with 2 DOFs each and in 3D, the hand has 5 fingers with 3 DOFs each.

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.2\textwidth]{figs/3d5fHand.png}
% \includegraphics[width=0.2\textwidth]{figs/2d4fHand.png}
% \caption{Left to right: an image of the 3D 5-finger hand,  and the 2D 4-finger hand}
% \label{hand_model}
% \end{figure}

% Successfully learning the task usually involves the following behaviors that we define here, as shown in Figure \ref{behavior}:
% \begin{enumerate}
%     \item Turning: Fingers move together to rotate the object with a constant angular velocity, without intentionally breaking contacts. 
%     \item Switching: A finger breaks contact from the object, then makes a contact at a nearby location on the object.
%     \item Sliding: A special case of switching where a finger moves its contact point on the object without significantly breaking it.
%     \item Gaiting: Fingers continuously switch and turn in a looped behavior to maintain constant rotation without dropping the object.
% \end{enumerate}



% \subsection{Finger gaiting In-hand manipulation}

% The goal of this problem is to rotate the object as much as possible around the ${z}$ axis (up-down), therefore the reward of each step is the angle change of the object around the ${z}$ axis with a penalty for tilting. Each episode ends if the maximum timestep reached or the object is lost (when number of contacts is less than the minimum number of contact).

% We have performed baseline experiments i.e SAC without guided exploration on 4 different settings so far: 6DOF cube  and 6DOF sphere in 3D 5-Finger Hand, 3DOF(${x}$, ${y}$ translation and ${z}$ rotation) round disk and 1DOF(${z}$ rotation) round disk in 2D 4-Finger Hand, as shown in Figure \ref{baseline_compare}. 
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.5\textwidth]{figs/baseline_comparison_legend.png}
% \caption{Baseline training curves (Episode Reward vs. Timesteps) of in-hand manipulation on different settings.}
% \label{baseline_compare}
% \end{figure}

% By rendering the policy saved in different timesteps, we discovered that the policy learns the behaviors turning, switching, and gaiting sequentially, as shown in Figure \ref{baseline_stage}. This is consistent for all settings except for the case 3D 5-Finger Hand with cube where the policy fails to learn finger gaiting. For the models that learn to gait, the timesteps of learning the behaviors described above vary, but all following the order of turning, switching, and then finger-gaiting.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.5\textwidth]{figs/baseline_sphere_stage.png}
% \caption{Learning progress of baseline on 3D Hand with a sphere object (Episode Reward vs. Timestep).}
% \label{baseline_stage}
% \end{figure}
